A Privacy-preserving Mobile and Fog Computing Framework to Trace and Prevent COVID-19 Community Transmission

To slow down the spread of COVID-19, governments around the world are trying to identify infected people and to contain the virus by enforcing isolation and quarantine. However, it is difficult to trace people who came into contact with an infected person, which causes widespread community transmission and mass infection. To address this problem, we develop an e-government Privacy Preserving Mobile and Fog computing framework entitled PPMF that can trace infected and suspected cases nationwide. We use personal mobile devices with contact tracing app and two types of stationary fog nodes, named Automatic Risk Checkers (ARC) and Suspected User Data Uploader Node (SUDUN), to trace community transmission alongside maintaining user data privacy. Each user's mobile device receives a Unique Encrypted Reference Code (UERC) when registering on the central application. The mobile device and the central application both generate Rotational Unique Encrypted Reference Code (RUERC), which broadcasted using the Bluetooth Low Energy (BLE) technology. The ARCs are placed at the entry points of buildings, which can immediately detect if there are positive or suspected cases nearby. If any confirmed case is found, the ARCs broadcast pre-cautionary messages to nearby people without revealing the identity of the infected person. The SUDUNs are placed at the health centers that report test results to the central cloud application. The reported data is later used to map between infected and suspected cases. Therefore, using our proposed PPMF framework, governments can let organizations continue their economic activities without complete lockdown.

==> privacy-preserving fog-mobile framework/abstract.tex <==
\begin{abstract}
% \Aron{move this sentence later (first describe the problem, then introduce the solution)}We present an e-government mobile and fog computing framework that can trace COVID-19 community transmission, while preserving user privacy. 
To slow down the spread of COVID-19, governments around the world are trying to identify infected people and to contain the virus by enforcing isolation and quarantine. However, it is 
% \Aron{why? would be good to provide an argument illustrating why the problem that you solve is challenging}
difficult to trace people who came into contact with an infected person, which causes widespread community transmission and mass infection. To address this problem, we develop an e-government Privacy Preserving Mobile and Fog computing framework entitled PPMF that can trace infected and suspected cases nationwide. We use personal mobile devices with contact tracing app and two types of stationary fog nodes, named Automatic Risk Checkers (ARC) and Suspected User Data Uploader Node (SUDUN), to trace community transmission alongside maintaining user data privacy. 
% Our system creates a unique encrypted reference code for each user's mobile device
% Each user's mobile device generates a Universally Unique Identifier (\Aron{UUID means this: \url{https://en.wikipedia.org/wiki/Universally_unique_identifier} is this what you are using? if not, change name to avoid confusion}UUID) 
Each user's mobile device receives a Unique Encrypted Reference Code (UERC) when registering on the central application. The mobile device and the central application both generate Rotational Unique Encrypted Reference Code (RUERC), which broadcasted using the Bluetooth Low Energy (BLE) technology.
%%%%Any nearby mobile device can receive the RUERC and record it for the next 21 days. %%%
%The application \Aron{how? receiver can choose to keep a plaintext copy if it wants to}maintains user privacy by storing the UERCs in an encrypted and \Aron{who sets the password? how do you prevent offline brute-forcing attacks? why is a password needed at all, why not just encryption with strong key?}password-protected folder that can only be accessed by the government.
% Government maintains the database of server-generated UERCs and contains a mapping between UERC and RUERC. 
% The users' mobile devices stores the RUERC in the application cache.
% without \Aron{why would we need encryption? it is not clear why this would be required without the central database}requiring further encryption.
The ARCs are placed at the entry points of buildings, which can immediately
% \Razon{Don't we need to address the number of person and time threshold in abstract?} \Shanto{I guess, no need, how we are not revealing the user identity is described later in main section}
detect if there are positive or suspected cases nearby. If any confirmed case is found, the ARCs broadcast pre-cautionary messages to nearby people without 
% \Aron{this might not be enough for privacy, e.g., if someone enters a building and the ARC goes off, it is obvious that the new person is the infected one}
revealing the identity of the infected person. The SUDUNs are placed at the health centers that report test result to the central cloud application. The reported data is later used to map between infected and suspected cases. Therefore, using our proposed PPMF framework, governments can let organizations continue their economic activities without complete lockdown. %Further, it becomes viable to identify superspreaders and to map the cluster of infected and suspected cases.
\end{abstract}




% Note that keywords are not normally used for peerreview papers.
\begin{IEEEkeywords}
COVID-19, Community Transmission, Contact Tracing, Mobile App, Data Privacy, Fog Computing 
%COVID-19 Tracing Graph
\end{IEEEkeywords}

==> privacy-preserving fog-mobile framework/sections/background.tex <==
\section{Background}\label{sec:background}
Contact tracing and isolation of cases are required to control infectious disease outbreaks, and the consequence depends mainly on government actions and citizen responses~\cite{hellewell2020feasibility}. Manual tracing is difficult and time-consuming in a pandemic situation, and governments are pushing for digital surveillance to contain the spread of the virus in the context of health informatics~\cite{BigDataHealth}.
% \change{}{ Shanto: can we cite this here: https://ieeexplore.ieee.org/document/7154395 ?}. 
However, these mobile apps have raised questions over user data privacy since digital surveillance involves location tracking, limits individual freedom, and expose confidential data~\cite{raskar2020apps}. 


\subsection{Contact Tracing}
% \itodo{write some statistics since the beginning}
% As of 24th May, 2020,  5,427,555  cases  of COVID-19 have been reported including 344417 deaths and 2,259,440 recoveries\cite{WM:online}  across 213 Countries and Territories around the world \cite{ecdc:online}. The most number of cases and death till date is found in the USA approx. 1,666,829 \cite{WM:online}. The USA and Brazil reported more than 10 million cases in the last 7 days \cite{whoreport:online}. On 14th March, 2020 in America, Asia, Europe and Oceania and the number was 1,42,534 confirmed (9764 new) 5,392 deaths \cite{WM:online}. In 70 days, the case has increased by almost 50 times. According to a recent report, 12.6\% cases are transmitted pre-symptomatic \cite{stat6}. Singapore and China have inferred pre-symptomatic transmission of around 48\% and 62\% respectively through modeling and estimation, in the presence of control measures \cite{stat7}.


% \paragraph{Quarantine:}
% If a person has already come in contact with a positive case, he needs to stay at home in quarantine.

% \paragraph{Isolation:}
% If a person is confirmed positive, he needs to isolate himself in a room or apartment from other people.

% \paragraph{Incubation Period}


% \subsection{Contact Tracing}
% \cite{cho2020contact}


Governments can stop transmission of COVID-19 if they identify cases and their contacts quickly and get them to limit their connections with other people. Cases should isolate themselves as long as they are infectious- for at least $10$ days after they became ill. Contacts must quarantine for $14$ days after the last contact with an infectious patient~\cite{pung2020investigation}.
% \Razon{Shouldn't we use reference for this information}. 
Some cases may have close contact with many people because of where they have been or where they live, and these situations should immediately be reported.

Contact tracing might be difficult as an infected case may not remember all people who came in their contacts. Additionally, an infected person may not know or remember the phone numbers and address of their contacts. It may take longer for authorities as well due to the required time to identify and get in touch with contacts. Therefore, mobile-based contact tracing might help track several contacts and determine who is at highest risk for infection. 

Contact tracing usually requires three primary steps: contact identification, listing, and follow-up~\cite{raskar2020apps}. People with contact with an infected person are considered as suspected cases if they were in proximal range for more than 15 minutes, within 6 feet~\cite{CDC:online} or the distance of more than 6 feet, but stayed nearby for an hour~\cite{COVID19C58:online}.

% Therefore, 
% 1)	Public health staff time is often limited specially in a pandemic situation.
% 2)	Timing of events is very important-we need to reach people quickly.
% 3)	Technology can improve efficiency and speed some of public heath frontiers
% 4)	Technology should meaningfully improve the process without creating major difficulties.

% Normal contact tracing ...SIX STEPS
% 1)	Introduce
% 2)	Enquiry
% 3)	Identify contact
% 4)	Issue Isolation
% 5)	Initial contact tracing
% 6)	Regular check in
% CONTRACT TRACING TOOLS protect the health of public.

% \cite{raskar2020apps} mentioned the following three steps for contact tracing-
% \begin{enumerate}[i.]
%     \item Contact Identification
%     \item Contact Listing
%     \item Contact Follow-Up
% \end{enumerate}

% \subsubsection{Tracing Suspected Cases}
% \begin{itemize}
%     \item more than 15 minutes
%     \item within 6 feet distance
%     \item distance more than 6 feet but nearby for an hour
% \end{itemize}

% \paragraph{exception:}
% A person is considered a suspected case, if he comes in contact with a confirmed case within more than 6 feet radius only if more than an hour.



%-------------------------------------------------
%---------------Related---------------------------
%-------------------------------------------------
\subsection{Contact Tracing Frameworks and Applications}
Due to the necessity of tracing infected or suspected cases, governments around the world have developed several tracing applications and frameworks~\cite{cho2020contact}. The most common features of these applications are live maps and news updates of confirmed cases, location-based tracking and alerts, quarantine and isolation monitoring, direct or indirect reporting, self-assessment, and COVID-19 education~\cite{sharma2020use}. Some governments involved third parties to develop such applications and encouraged citizens to use these applications. 

% Drew et al. presented a mobile application entitled \snippet{COVID-19 Symptom Tracker}~\cite{drew2020rapid}.

% Privacy concern- DHT - \cite{brack2020decentralized}.




%----------------------------------------------------------------------
%-------------------------- ISSUES-------------------------------------
%----------------------------------------------------------------------
% \subsection{Issues of Existing Works}
% Applications have several design consideration issues, tracing incorrectness, and most importantly privacy-oriented issues~\cite{Afloodof14:online}.
% Here, we discuss several issues we have traced so far.
% \vspace{2mm}
\subsubsection{Privacy Concerns}
Since governments have been rushing to build tracing applications, the least they have considered about user data privacy. In most cases, users can be monitored and tracked in real-time without user’s consent. If such mobile applications store the location history, user movement can be traced as well~\cite{berke2020assessing}. Apart from location tracking, there are several other user privacy issues, such as excessive data collection, obscure data flow, lack of user control, and data usage policies.

% % \paragraph{Geo-location tracing:}
% \paragraph{Mobile App Design Considerations:}
% \Aron{MIT Tech Rev is a magazine, name the authors instead}MIT Technology Review
Abeler et al.\ suggested that we can achieve contact tracing and data protection at the same time by minimizing data processing in the existing frameworks~\cite{abeler2020covid}.
However, many applications are not following such solutions and Howell et al.\ has suggested five primary privacy concerns for COVID-19 application frameworks~\cite{Afloodof14:online}.
    \begin{itemize}
        \item \textit{Voluntary or Mandatory:}
        It should be a voluntary act whether users download and use such tracing apps. With the growing concern over data privacy, unnecessary data collection, location tracking, and other issues, users must have free wills to decide. The government or any third party cannot mandate users to use these apps in any circumstances.
        \item \textit{Data Usage Limitation:}
        People are concerned over the collected data usage for personal safety reasons~\cite{simko2020covid}. Therefore, the collected data must have usage limitations. For example, tracing data can only be used for public health and safety. Traced data cannot be used for any other purpose, e.g., law enforcement.
        \item \textit{Data Destruction:}
        Mobile applications or a framework should automatically delete user records after a particular period~\cite{dubov2020value} (e.g., usually 14-21 days and no longer than 30 days). Otherwise, users should have manual control over data deletion from the app or the central server.
        \item \textit{Minimal Data Collection:}
        Several applications collect excessive, unnecessary data from its users, for example, an application named
        \snippet{Aarogya Setu} requires name, phone number, age, gender, profession, and details of countries visited in the last 30 days.
        % \change{}{ Shanto can we cite shorturl.at/bnouO}. 
        Also, Geo-location tracing is unnecessary alongside Bluetooth or other similar wireless technologies~\cite{Microsof7:online}.
        
        \item \textit{Transparency:}
        The entire process of data collection and usage should be transparent to preserve user privacy. Application frameworks should have publicly available policies, clear and concise data flow and database, and open-source codes for transparency. Additionally, users should have full control over their data usage. Therefore, developers must follow the \emph{compliance} and \emph{consent} rules (GDPR, HIPAA, CCPA, etc.) strictly~\cite{GDPRCompliance,dubov2020value}.
        
    \end{itemize}


Apart from the privacy issues mentioned above, there are certainly other things to consider, as well. For example,
the mobile application generated IDs can be breached, decrypted, and resulted in exposing user information. Additionally, applications controlled by the third party may pose a severe threat as they can misuse the collected user data. Therefore, in terms of privacy, user control over the owner's data and transparency are notable factors.


% \paragraph{Compliance and Consent:}

% \paragraph{User data deletion policy:}
%         \begin{itemize}
%             \item User can't delete data from app or server
%         \end{itemize}
    


\vspace{2mm}
\subsubsection{General Concerns}
Apart from several data privacy issues, different design issues are prevailing in the contact tracing apps. Many applications require a constant internet connection while it is entirely unnecessary. In some other implementations, the user can not turn off the background service of the apps, and these apps do not feature turn-off option.
% \Shanto{need reference}. 
The apps continue to work at random times, such as while staying at home or sleeping. Therefore, it causes battery drains too fast.

Tracing correctness depends on the distance and period of contact. Several applications stores the RUERC of a nearby user device even there is a wall between two persons. Moreover, rushing to develop such applications result in \emph{false positive} suspected victim considerations and community transmission. Communication between multiple platforms may appear troublesome and can lead to unexpected behavior. Therefore, using Google/Apple API might be helpful to introduce Bluetooth communication between two devices of different platforms (Google Android and Apple iOS). Apart from these issues, \emph{insecure source code}, \emph{weak data flow and process}, and different \emph{Bluetooth-based device attacks} can cause security hazards. 



% \vspace{2mm}
\subsubsection{Google/Apple Exposure Notification API}
% \Razon{Sir, Shanto vai, Shovon vai, please check if this is okay}
%{Checked already.........WZ}
Google and Apple announced their privacy-preserving exposure notification in April 2020 and released phase one in May 2020~\cite{ExposureFAQ42:online}. The API uses BLE technology and applies different hashing algorithms to generate different keys on a specific time interval~\cite{ExposureBS20:online} to prevent wireless tracking. Infected cases upload only the daily generated keys of the past 14 days, and other users download lists of these keys of infected cases of their corresponding region. 

All the key-generation and risk-level checks are performed in the user's mobile device, preserving user privacy. However, this might also be a concern about the resource consumption of that particular mobile device~\cite{HashEC}. Moreover, as the user is only uploading their keys, the authority can not notify the contacts of the infected case immediately. Some other essential functionalities, such as preventing community transmission and identifying the asymptomatic spreaders, can also be troublesome.

The responsibility of implementing this technology is on the corresponding public health authorities. However, the authority is required to follow the guidelines of privacy, security, and data control rules as well as the development criteria such as file and data format of storing, uploading, and downloading keys~\cite{ExposureFAQ42:online,ExposureTerm72:online}.
This collaborative development of the Exposure Notification ensures that both the platform (Android and iOS) transmits and receive similar keys, and the risk level the app calculates is also similar.

% Google and Apple announced their privacy-preserving exposure notification in April 2020 and released phase one in May 2020~\cite{ExposureFAQ42:online}. The API provides functionality to use Bluetooth technology to trace the contacts. The Bluetooth transmits an encrypted Associated Encryption Metadata (AEM), which includes the Rolling Proximity Identifier (RPI)~\cite{ExposureBS20:online}. This RPI is generated from a Temporary Exposure Key (TEK) every 15 minutes interval to prevent the wireless tracking of the system. The API uses HKDF, RPI key, and AES from interval number at the time of the Bluetooth Mac address changes to generate RPI and  HKDF, AEM key, and AES-CTR from Bluetooth metadata to generate AEM.

% While installing the application, the API generates a Unique key that stays in the device, and from this key, the API generates TEK on 24 hours interval. When a person comes in proximity to another person, they broadcast and save the RPI. The user will upload the set of TEK of the past 14 days to the cloud if found positive. The API downloads this case list once a day and notifies the user about the user's risk level. The risk level depends on whether the user was in contact with any positive case and the duration they have spent together~\cite{COVID19C58:online}.
% The API prevents wireless tracking and preserves the privacy of the user. Development of the application is the responsibility of the authority, but to implement these APIs, they must abide by the provided rules and regulations. However, there is hardly any way to backtrack a case that may make some preventions more troublesome.

% \begin{itemize}
%     \item \textit{Preventing community transmission:}
%     The user can check the risk level once a day. After checking, the user can be infected at any time of the day and becomes contagious for the people who comes in contact with, for the rest of the day. Moreover the authority of the places the user visited do not have any alert system.
%     \item \textit{Notifying suspected contact users:}
%     The case is only uploading his/her daily TEK of the past 14 days, not the contacts the case came close. Therefore, authority can not notify the suspected contacts immediately. 
%     \item \textit{Identifying super spreader and cluster:}
%     There might be some people who are not facing any symptoms but spreading the virus. Singapore and China have inferred pre-symptomatic transmission of around 48\% and 62\% respectively through modeling and estimation, in the presence of control measures~\cite{stat7}.
% \end{itemize}

% We find the \emph{Exposure Notification API} preserves user privacy to the very end. However, there are a few other issues that require the proper solution:
% \begin{itemize}
%     \item \textit{Resource consumption:}
%     The API executes hashing to generate RPI on 15 minutes interval. It executes hashing to generate the RPIs of the past 14 days of each case from the case list downloaded from the server ~\cite{ExposureCS33:online}. This large number of hashing computation can be a concern for mobile devices~\cite{HashEC}.
%     %The API is generating RPI on 15 minutes interval by executing several hashing algorithms. Therefore, a device is required to execute hash algorithms 96 times a day. Additionally, when a user downloads the list of cases, it requires generating all the RPIs of each user from the past 14 days~\cite{ExposureCS33:online}. For a specific user, it is required to perform the hash algorithm 13.44 thousands of times. If there is a 10 thousand case in a list, it has to perform 13.44 million hashes. There will be 13.44 million RPI keys as well that need to be searched with the contact list of the user. This huge amount of computation is certainly a concern for a mobile device~\cite{HashEC}. \Shanto{use-> requires massive computation at the server end (for example, it may require computation if the considered generation of keys in every 15 minutes)} \Razon{The Computation actually happening in mobile end}
    
%     \item \textit{Accuracy on identifying contact:}
%      According to CDC \cite{CDC:online}, a person is \emph{contact} if he/she stays close to a \emph{case} for 15 minutes, within 6 feet distance, and according to Emily Gurley~\cite{COVID19C58:online} it requires 1 hour for a person who is nearby. The RPI is generating on 15 minutes interval. Therefore,  multiple RPI can be generated for a single person within this time frame. Also, identifying the correct RPI can be less accurate, and storing all the nearby RPI  may impact on device memory.
%     %According to CDC \cite{CDC:online}, a person is contacted if he/she stays close to a case for 15 minutes, within 6 feet distance. The RPI is generating on 15 minutes interval. Therefore, there is a possibility that a user may come in close with another person for more than 10-15 minutes after generating a key that results in broadcasting and storing two different RPI for one user. Hence the time spent together is not calculated correctly. Furthermore, a person is considered a contact if he/she is within the range of Bluetooth of the case for an hour~\cite{HomeJohn79:online}. The Exposure Notification API does not clearly state the filtering methods.
% \end{itemize}

% We adopt the theory of generating RPI on a specific time interval to prevent wireless tracking.

Current contact tracing apps backed by the governments have numerous design and privacy issues due to the rush for community transmission tracing. Regardless of addressing existing issues, the question remains if the governments can continue the economic activities alongside. Therefore, our integrated mobile and fog computing-based framework can solve the issues by effectively tracing community transmission while organizations can run their economic activities. 

==> privacy-preserving fog-mobile framework/sections/conclusion.tex <==
\section{Related Work}\label{sec:related}
% \Shanto{Please, suggest a few Privacy Preserving frameworks}
% \Shanto{Not finalized. Just random contents for now.}
Qiang Tang discussed a few existing privacy-preserving framework solutions that attempted to solve several user data privacy issues~\cite{tang2020privacy}. Author provided some observations and privacy solutions on Singapore's \snippet{Tracetogether}, Reichert et al.’s \snippet{MPC Solution}~\cite{cryptoeprint:2020:375}, Altuwaiyan et al.’s \snippet{Matching Solution}~\cite{altuwaiyan2018epic}, and Vaudenay's \snippet{DP3T} solution~\cite{cryptoeprint:2020:399}.

% \vspace{1.5mm}
\paragraph*{Singapore's Tracetogether}
Affected users are compelled to share with the Ministry of Health the locally saved information. In our framework, this is voluntary to share any information with the system.
Additionally, there is a risk of decomposition of the app and collecting the geo-location data from the app. As we are not storing any geo-location data anywhere, this does not possess any risk of transpassing. 


% \vspace{1.5mm}
\paragraph*{Reichert et al.’s MPC Solution}
This solution requires the user’s smart device to be used to acquire and save geo-location data, and this location trace is shared with the Health Authority (HA)~\cite{cryptoeprint:2020:375}. This may raise a privacy issue of the users as it does not mention if they can preserve their privacy by controlling what information they want to share with the authority and what information they do not want to share. 
We provide a clear and concise privacy dashboard to the users so they can choose the information they want to share and alter their choices.
The solution does not consider the scalability of computation of extensive data set collected from the devices, and HA requires to arrange garbled circuits (a cryptographic protocol that encrypts computation) for all infected users. We take precautionary steps in fog nodes to filter the collected data. Additionally, the central application uses an auto-scaling technique and a queue service to facilitate the upcoming data.


% \vspace{1.5mm}
\paragraph*{Altuwaiyan et al.’s Matching Solution}
This solution utilizes a privacy-preserving matching protocol between users along with proper distance measuring procedure~\cite{altuwaiyan2018epic}. We are using similar metrics to calculate the distance between mobile devices. On the other hand, infected users' exact location is shared with the central server, which indicates severe privacy violation. We do not use individual users’ locations and thus preserve users’ location privacy.


% \vspace{1.5mm}
\paragraph*{The DP-3T Solution}
The DP-3T solution provides a privacy-aware framework while considering three design considerations: low-cost design, unlinkable design, and hybrid design. The solution takes advantage of the content delivery network and provides a cost estimation per patient. Authors discussed privacy concerns such as the social graph (social relationships between users), interaction graph (physical interaction nearby), location traceability (tracing individuals), at-risk individuals (suspected cases), positive status (infected cases), and exposed location (partial identification of places a positive case visited). They also discussed the addressable privacy concerns in terms of the three design considerations.

\paragraph*{COVIDSafe}
The app collects user name, phone number, age-range, and postcode followed by the consent of the user and sends to the server. The app stores encrypted user ID, time of contact, and Bluetooth signal strength and keeps this data for 21 days. The case can upload these data voluntarily~\cite{CovidSafePrivacyp9:online}. The government has amended the Privacy Act 1988 to prevent the misuse of these data~\cite{CovidSafePrivacyA5:online}. The user can uninstall the app to delete these data and to delete all data from the server, the user needs to wait until the pandemic is over whereas, our framework allows users to delete all data within 14 days. 
% They trace the user with ID and alerts the contact with their phone number. However, the reason for collecting names, age-range, and postcode is not clear yet.


% \Shanto{I'll write a discussion here on the difference between existing solutions and our solution}

Table~\ref{tab:comparison} presents the difference between existing mobile application frameworks and our integrated mobile-fog computing framework (PPMF). Here, we categorize different features in terms of privacy-preserving approaches (voluntary, data usage limitation, data destruction, minimal data collection, and transparency), fog-based integrated solutions (risk check, infected/suspected data upload), and general design approaches (temporary BLE IDs, no geo-location trace, and minimal internet requirements). % We put \emph{checkmarks} (\checkmark) to identify if a feature is present in any of the mentioned frameworks included in the first column.
We put our framework (PPMF) at the end of the list and find it ticks all these features.

\input{tables/comparison}

\balance

\section{Conclusions}\label{sec:conclude}
In this work, we have presented a mobile and fog computing-based integrated framework that can trace and prevent community transmissions alongside maintaining user data privacy. In \emph{PPMF}, we consider minimal data collection and provide a temporary RUERC in encrypted form for storing in user devices. 
% The central cloud application generates the UERCs and provides a registered user. 
The \emph{ARC} is responsible for tracing positive cases in public places and sending alerts to nearby people without revealing the user's identity. The \emph{SUDUN} uploads data to the central database about infected and suspected cases that can be processed to identify a super spreader and visualize the clusters of cases based on postal codes and age groups.

Minimal and undetectable data collection, user control, and system transparency are essential factors to ensure user data privacy. Privacy dashboard-based on compliance and user consent makes it convenient and encourages citizens to use such a user-friendly e-government framework. Therefore, using the structure of our proposed \emph{PPMF} framework, governments can continue their economic activities while tracing and minimizing the mass-level community transmission. In the future, we plan to develop a super spreader detection model and clustering methodology of infected cases, based on our  framework.






\section*{Acknowledgement}
This research is partly supported through the Australian Research Council Discovery Project: DP190100314, 'Re-Engineering Enterprise Systems for Microservices in the Cloud.'

==> privacy-preserving fog-mobile framework/sections/development.tex <==
\section{Framework Development} \label{sec:development}
In this section, we discuss the implementation overview of our framework with regards to \emph{Amazon Web Service}. Additionally, we discuss the database design, analysis of our contact tracing graph, and our privacy-preserving solutions.

\subsection{Implementation Overview}
We have implemented our framework using Amazon Web Services (AWS)~\cite{robinson2008amazon,AmazonWe40:online}. As it is a generic framework, it can be applied in other IoT/Cloud platforms too. The fog nodes, ARC and SUDUN, consist of AWS Greengrass components and Lambda functions. They are connected to the AWS IoT Core service using the MQ Telemetry Transport (MQTT) protocol. The authenticity and security of the fog nodes are ensured by using IoT Device Defender. IoT Device Management service is used to monitor and audit the fog nodes. Incoming data from the fog nodes are passed to Simple Queue Service(SQS). The queue data is processed via Lambda functions and moved into the application containers, which is managed via the Kubernetes cluster within an auto-scaling group for dynamic scaling of the master nodes and worker nodes.

After the data is processed in the application nodes, it is sent to the Redis Cache tier and eventually to the Amazon Relational Database Service (RDS). For the administration of the cloud application, an SSH connection is provided via Elastic Load Balancing to a Bastion server. The users need to be connected to the cloud application only on the registration process via HTTPs connection to a load balancer. The test centers send the test results using RESTful API over HTTPs. The scheduled tasks, for example, generating the user's rotational UERC, is done in an Elastic Container Service, which uses the CloudWatch event rule at a specific time of the day. The application generates alarms for any irregular activities like device connection error or access failure via CloudWatch alarms to the proper authority. Users are notified from ARC, SUDUN, and cloud application via Simple Notification Service. For further communication processes to authorized organizations and administrators, the Simple Email Service is used. For restricting unauthorized access to the applications and data layers, private subnets are used. To ensure efficient data availability in the cloud, a database instance is stored in a separate availability zone. Here, Figure~\ref{fig:Implementation Overview} illustrates the implementation overview.


\begin{figure*}[!ht]
    \centering
    \includegraphics[width=.87\textwidth]{figures/architecture.pdf}
    \caption{Implementation Overview with regards to AWS}
    \label{fig:Implementation Overview}
\end{figure*}


\subsection{Database}
The cloud database includes several tables to trace infected and suspected cases, to alert users, to prevent community transmission in organizations through ARC, and collect test results from SUDUN. The user table stores user registration information (mobile number, age group, postcode, and timestamp) and the initial UERC. As we are generating new UERCs associated with the primary user UERC, we need mapping in between those unique reference codes. We store test results (result ID, test organization ID, timestamp, test result, and user mobile number) in a separate table and extract the infected users (affected UERC, test result ID, and affected ID). Now, we map between the registered user table and affected user table to find out the suspected users and store the suspected UERC, duration, timestamp, and distance radius alongside generating a new suspect ID. We also need an organization database where we store organization information (name, email, geo-location, address.) and associated permissions for ARC and SUDUN. Figure~\ref{fig:database_tables} presents the relations between all these tables.
% \begin{itemize}
%     \item Users: It stores registered users public information. Each properties are stored only after getting consent from user. The properties are: UERC(pk), mobile\_number, age\_group, postal\_code and added\_at
%     \item UERC\_Mapper: It stores generated UERC for each user for 14 days. The generated UERC is mapped with the original UERC and generated UERC which are older than 14 days will be overwritten. The properties are: mapper\_id(pk), user\_uerc(ok), and generated\_uerc
%     \item Permissions: It stores the permission list which will be used by various types of organization. The properties of this table are: permission\_id(pk), permission\_title
%     \item Organization\_Types: To distinguish the permission level from one organization from another, this table is created. The properties are: organization\_type\_id(pk), organization\_type\_title
%     \item Organization\_Permission: It is a connecting table for Organization\_Type and Permissions table that stores what permissions are listed for each type of organization. The properties are: organization\_permission\_id(pk), organization\_type\_id(fk), permission\_id(fk)
%     \item Organization: It stores information about each organization. To identify each organization's accurate location, latitude and longitude of each organization are stored. The properties are: organization\_id(pk), organization\_type\_id(fk), parent\_organization\_id(fk), name, email, phone, address, latitude, longitude, password, added\_at, status
%     \item Test\_Results: It stores each test results including positive and negative results and are mapped using mobile\_number attribute of the user. The attributes are: test\_result\_id(pk), test\_organization\_id(fk), result\_timestamp, test\_result, mobile\_number
%     \item Affected\_Users: It stores only information about affected users. The attributes are: affected\_id(pk), affected\_UERC(fk), test\_result\_id(fk)
%     \item Suspected\_Users: This table stores information about only the suspected users. The attributes are: suspection\_id(pk), affected\_id(fk), suspected\_UERC(fk), added\_by\_organization\_id(fk), duration, connection\_timestamp, distance, added\_at

% \end{itemize}

\begin{figure}[!ht]
    \centering
    \includegraphics[width=.5\textwidth]{figures/covid_erd.pdf}
    \caption{The cloud database consisting of mandatory tables}
    \label{fig:database_tables}
\end{figure}






\subsection{Contact Tracing Graph}
To identify and trace COVID-19 community transmission, we introduce and utilize a graph database called \snippet{Neo4j}~\cite{Neo4jGra88:online} to determine the contact graph. 
Figure~\ref{fig:contact_tracing_graph} presents a portion of the contact tracing graph with synthetic data of contact tracing. The red, blue, and green circles indicate the test centers, users, and test results. The lines present directed edges of the graph between infected and suspected victims.
The tracing graph can be used to identify individuals who had come in close contact with infected victims almost in real-time. We can determine a potential super spreader as well, using the contact tracing graph. Additionally, suspected victims identified by the graph can be informed to take cautionary actions to prevent community transmission.


\begin{figure*}
    \centering
    \includegraphics[width=.94\textwidth]{figures/clustering.png}
    \caption{Contact tracing graph}
    \label{fig:contact_tracing_graph}
\end{figure*}





\subsection{Privacy Preservation}
As we discussed five major data privacy issues earlier in Section~\ref{sec:background}, here, we discuss solutions to these issues in terms of implementing our framework. 


% \vspace{1.5mm}
\subsubsection{Voluntary} 
Users have full control over the usage of this application and the stored data in the application storage. Even it is an e-government framework, no one can force users to use the mobile app, and the participation is voluntary. While using the mobile application, users have a privacy dashboard (Figure~\ref{fig:user_privacy_dashboard}) where he can allow if the app wants to store collected RUERCs in the local storage, use device Bluetooth to share user's RUERC, and if the user wants to share the collected RUERCs with the government.



     
% \begin{figure}[!ht]
%     \centering
%     \includegraphics[width=.4\textwidth]{figures/privacy_dashboard.PDF}
%     \caption{User Consent Privacy Dashboard}
%     \label{fig:user_privacy_dashboard}
% \end{figure}

% \vspace{1.5mm}
\subsubsection{Minimal Data Collection}
Initially, the system collects the user's \emph{age group}, \emph{postal code}, and \emph{mobile number} for registration and, in return, provides a unique ID (UERC) to be stored in a user's mobile device. Then the mobile application collects \emph{RUERC}, \emph{timestamp}, \emph{duration}, and \emph{distance} measure (based on RSSI) from other mobile devices that came in contact with the user's device. Age group and postal code are optional fields. These fields are used to define clusters and identifying super spreaders. The phone number is used to alert contact to take precautions. No personal information of the user is collected during or after the registration procedure. Figure~\ref{fig:registration_minimal_data} presents the mobile application user interface with mandatory and non-mandatory fields.

% \begin{figure}[!ht]
%     \centering
%     \includegraphics[width=.4\textwidth]{figures/registration-covid.PDF}
%     \caption{Minimal Data Collection during Registration}
%     \label{fig:registration_minimal_data}
% \end{figure}

\begin{figure*}[t]
\centering
\begin{subfigure}{.37\textwidth}
  \centering
  % include third image
  \includegraphics[width=\linewidth]{figures/privacy_dashboard.PDF}  
  \caption{User Consent Privacy Dashboard}
  \label{fig:user_privacy_dashboard}
\end{subfigure}
\begin{subfigure}{.37\textwidth}
  \centering
  % include fourth image
  \includegraphics[width=\linewidth]{figures/registration-covid.PDF}  
  \caption{Minimal Data Collection during Registration}
  \label{fig:registration_minimal_data}
\end{subfigure}
\caption{Privacy Concerned Mobile Application User Interfaces}
\label{fig:fig}
\end{figure*}


% \vspace{1.5mm}
\subsubsection{Data Destruction}
The mobile application deletes collected RUERCs no later than $21$ days calculated from the latest timestamp. In the cloud application, UERC and associated data from the suspected table is deleted in $30$ days of entry timestamp. Additionally, a user has full control over his data and can delete it manually from the application storage instantly. A user can also request for account deactivation and deletion of data from the cloud database. However, it may take up to two weeks to synchronize data in all replica databases.


% \vspace{1.5mm}
\subsubsection{Transparency}
Transparency is vital in data privacy, and governments should make the source codes open and publish the user data flow in the whole framework. Transparency motivates users to use an application and results in better management and increased public engagement. Consent and compliance can play a crucial role in presenting transparent data processes and improving decision making. 


% \vspace{1.5mm}
\subsubsection{Limited Data Usage}
The collected data should have limited use cases, and our framework opens the opportunity to determine a \emph{super spreader}, and \emph{clustered view} of positive cases. Additionally, the infected and suspected lists can help calculate the risk factors in terms of community transmission. However, while employing, further data usage should be minimal, and users need to have a clear idea of why and how data is being processed.




==> privacy-preserving fog-mobile framework/sections/introduction.tex <==
\section{Introduction}\label{sec:intro}

% We are passing now a pandemic that normally occur once in a 100 years. This is very unprecedented and global act which affect all the nations and country worldwide. 
% Since, this diseases is caused by SARS virus COVID2 and named as a COVID19.
% The COVID-19 pandemic has caused 
% In this pandemic, when human life is in danger, researchers come forward different tools  and technology to fight with COVID19. In this consequences, mobile based apps and digital technology is introduced currently to tackle the the number of infectious people recently. As we understand, the reducing of affected people, confirmed case can dramatically subsidized the unprecedented growth of pandemic. Therefor, digital technology plays a vital role to contact tracing and isolate people and reduce the spread of the virus drastically.

% Accordingly, as we said earlier, contact tracing is a vital part of this disease management perspective. Therefore a number of tools already come to the market and used by the different companies worldwide. However, recent surveys show that most of the tools, digital technology violates the privacy and personal data and human rights. In this circumstances, we strongly feel that a privacy protective framework or guide lines by maintain the WHO guide lines and personal data protection and privacy aware digital technology is a must.

% In this research, we design and develop a Fog cloud based privacy aware contact tracing framework by using mobile apps. We introduce the working principal, registration process of contact tracing apps. In addition, we design the Fog node and cloud based database server to collect the apps data and find the contact digitally and isolate a/quarantine with using technology. Moreover, we discuss several use case scenario, such as personal risk assessment, Automatic risk checker in different use case. Further more, we ensure our contact tracing framework compiling the  privacy and data protection compliance aware framework. Finally, we show the key privacy criteria are passed by our Framework. All these aspects, we finalize several research questions and map these answers in our research. 

\IEEEPARstart{T}{he} novel corona virus disease in 2019 (COVID-19) has spread rapidly
worldwide in a short duration. It caused a significant public health crisis worldwide, and by the end of May 2020 (i.e., within the five months of its first infection detection), over $6.16$ million persons were infected, and over $372$ thousand have died~\cite{HomeJohn79:online}.
Therefore, governments worldwide seek solutions to minimize the infected cases from the COVID-19 pandemic by employing mobile application based contact tracing~\cite{sharma2020use,chan2020pact}. Mobile apps can help trace both infected and suspected cases in almost real-time, and governments are rushing towards developing and deploying such applications and frameworks. However, several applications raise significant privacy issues as they collect sensitive and personally-identifiable data from users, and lack user control and transparency in data processing or usage~\cite{sharma2020use,cho2020contact,chan2020pact,raskar2020apps}.

Governments are enforcing temporary lockdowns of cities to slow down the spread of COVID-19, causing tremendous economic losses. However, we can alleviate economic impact by avoiding wide-scale lockdowns and performing more targeted isolation.
% \Aron{need to connect these two sentences better: add a sentence here clarifying that we can alleviate economic impact by avoiding wide-scale lockdowns and performing more targeted isolation}
Therefore, introducing fog computing in economic zones (e.g., shopping malls, organization buildings) can ensure continued economic activities by alerting nearby people while mobile computing (mobile apps) can help to trace the infected and suspected cases. However, to the best of our knowledge, there is 
% \Aron{need to be more specific here, there are app-based solutions for contact tracing that provide some level of privacy (I guess the key difference is the integrated framework, but it is not clarified here what that is)}
no integrated fog computing framework alongside contact tracing mobile apps that allows tracing community transmission while preserving users' data privacy. Therefore, we introduce the following research questions to find an appropriate solution to the cause.


% \paragraph{Research Questions:}
\begin{itemize}
    \item[\textbf{Q1.}] \textbf{Background and Issues:} What are the issues and privacy concerns in existing contact tracing apps?
    \item[\textbf{Q2.}] \textbf{Mobile and Fog Computing:} How to utilize mobile and fog computing to trace and prevent COVID-19 community transmission?
    \item[\textbf{Q3.}] \textbf{Privacy-preserving Framework:} How to develop an automated privacy-preserving e-government framework?
\end{itemize}

We answer the first question by looking into the background and issues of existing application frameworks as well as user data privacy concerns (Section~\ref{sec:background}). We find that there are several mobile application frameworks developed by governments and third parties to trace the COVID-19 community transmission. However, most of these applications and frameworks have failed to ensure user data privacy and suffer from other issues, such as mandatory use of apps, excessive data gathering, questionable transparency of source codes and data flow, unnecessary data usage or processing, and lack of user control in data deletion.

We answer the second question by presenting the design considerations, architecture, and workflow of our e-government application framework that utilizes mobile and fog computing (Section~\ref{sec:method}). The system consists of two types of fog nodes (ARC and 
% \Aron{need to introduce acronym before using it}
% \Aron{why are ARCs mentioned in the abstract but not SUDUN? are ARCs more important?}
SUDUN), several RESTful APIs, and a central application. Users can register themselves using User API. The ARC is used to check the risk of users visiting any public places (e.g., shopping mall, organization building). Test centers send the COVID-19 test results using Result API to the central application. If the test result is positive, then the user is requested to upload locally stored contact tracing information to the cloud using SUDUN or directly from mobile app. Figure~\ref{fig:block} presents an overview of the proposed system.

% We answer the third question by elaborating module development and implementation of our privacy-preserving framework (Section~\ref{sec:privacy}).

\begin{figure*}
    \centering
    \includegraphics[width=.7\textwidth]{figures/block_dia.pdf}
    \caption{System Overview}
    \label{fig:block}
\end{figure*}


We answer the third question by discussing the implementation overview and user data privacy solutions in our framework (Section~\ref{sec:development}). Here, we discuss the framework development based on the Amazon Web Services (AWS) solutions. Then we present the privacy preservation based on user control (voluntary, compliance, and user consent), minimal data collection (mobile number, postal code, and age group), data destruction at user's will, transparency (open source codes, clean data flow), and limited further usage of data.



% \paragraph{\textbf{Research Contribution:}}

% \begin{itemize}
%     \item We design a privacy-preserving Mobile and Fog computing framework that can trace and prevent COVID-19 community transmission nationwide
%     \item We have developed the contact tracing framework in such a way that it can provide a base headstart for future mobile applications endeavored by Governments, necessary in a Pandemic situation
%     \item Our developed system can effectively fulfill our objectives while consuming less power in both resourceful or resource-limited Cloud-IoT ecosystem
    
% \end{itemize}

% \vspace{2mm}
\paragraph*{\textbf{Scope}}
We intend our framework to be 
% \Aron{`deployed'? does it still need development?}
deployed and controlled by the central government of a country. 
Governments have access to the test results and can control such an integrated mobile-fog computing framework. 
Moreover, relying on a private entity
% \Aron{BTW, many consider sharing data with government to be just as bas as sharing with a private entity} 
to manage such a framework can limit the preservation of data privacy. 
Additionally, in this work, we primarily consider and focus on user data privacy issues. 
Regardless of building a standard and secure data processing framework, we do not discuss 
% \Aron{why? perhaps state that there is a rich literature on existing security measures and refer the reader to it} 
advanced security threats related to mobile, fog, and cloud layer as there are rich literature on existing security measures~\cite{roman2018mobile,yi2015security,singh2016survey}.


% \vspace{2mm}
\paragraph*{\textbf{Outline}}
The rest of the paper is organized as follows: Section~\ref{sec:background} introduces the privacy and general issues of existing contact tracing frameworks. Section~\ref{sec:method} discusses the design considerations, system components, and workflow of our proposed e-government framework. Section~\ref{sec:development} presents the implementation overview and privacy-oriented solutions of the framework. Finally, Section~\ref{sec:related} discusses a few related privacy-preserving frameworks followed by a conclusion.

==> privacy-preserving fog-mobile framework/sections/method.tex <==
\section{Framework Design}\label{sec:method}
% \itodo{Please suggest topics/subsections to add}
Our proposed privacy-preserving e-government framework has four major components: user mobile device and two types of fog nodes (ARC and SUDUN), and a central cloud application that integrates these nodes. Mobile Unit consists of BLE, privacy dashboard, filter algorithm, file storage, and communication service. A user mobile device advertises it's own RUERC, scans for RUERCs of other nearby devices, and save the filtered RUERCs (see filtering Algorithm~\ref{algo:suspect_filter}) in the file storage. 
% \Razon{Shanto vai, please review this starter passage}
%Privacy Dashboard contains all the information that the user has allowed the framework to do. Each operation, such as registration, advertising UERC, sending the file to SUDUN, etc. need to be approved by this Privacy Dashboard. 

Fog-based IoT-healthcare provides optimization of data communication, low power-consumption, and improves efficiency in terms of cost, network delay, and energy usage~\cite{mahmud2018cloud,IoTCloud}. 
The BLE in the ARC and SUDUN advertises a specific predefined UERC, and the mobile unit does not save these UERCs to file storage. When the user is in proximity to ARC (hospital, shopping malls, office), BLE of the ARC receives all the RUERCs around, and the fog component checks if there is any infected or suspected case. The cloud application responds with a positive or negative result without disclosing the victim's identity. If there is a positive case, the ARC transmits another predefined UERC that signifies the risk level and alerts all the mobile units around, including the infected or suspected case, hence preserving the victim's privacy. The other fog node, SUDUN, is set either in the test centers or where the authority finds it necessary. When the mobile unit receives the predefined UERC from this fog node, it checks its privacy dashboard. If the privacy dashboard allows the mobile unit to send the file to SUDUN, the mobile unit establishes a connection with SUDUN and send the file. Then, the fog component in SUDUN transfers the file to the corresponding cloud.
Here, 
% \Aron{how is this related to Figure \ref{fig:block}?}
Figure~\ref{fig:mobile_fog_framework} presents the detailed workflow our proposed integrated mobile and fog computing framework.


\begin{figure*}[!ht]
    \centering
    \includegraphics[width=.78\textwidth]{figures/PrivacyFramework.pdf}
    \caption{Mobile and Fog Computing Framework for Tracing and Preventing Community Transmission}
    \label{fig:mobile_fog_framework}
\end{figure*}


% \subsection{Concerns and Considerations}
% \subsubsection{Design Considerations}


\subsection{System Features}
We introduce the following features of mobile application and fog nodes in our integrated framework:

\begin{enumerate}
    \item \textit{Contact Tracing:} An user gets a hashed unique reference code upon registration from the system. Every two hours, another unique reference code is generated in the application, which is being shared with nearby devices upon user consent. It ensures that the broadcast data cannot be used to trace an individual. The same hashed value will be generated in the cloud application, and it can be used to check the risk level of any individual without disclosing his or her identity with others. 
    \item \textit{Self-checking:} Users can check if he or she was nearby any infected victim in the last 14 days using the mobile application. The application will upload the locally stored reference codes of the device it came in contact in the last 14 days. The cloud application will check if any of the uploaded RUERC is listed as an infected victim or suspected victim. The application will notify the user accordingly.
    \item \textit{Minimum Mobile Computation:} 
    Our proposed framework ensures minimum computation by enabling user control to turn on or off scanning, and background services. Apart from that, the mobile application features delay broadcast by avoiding unnecessary frequency and requires minimum internet connection as users only need internet while registering and uploading data for self-check.
    \item \textit{User Data Privacy:} User personal data is not stored or shared in the system. We ensure minimum data collection and avoid user location tracking or digital surveillance. Fog nodes do not identify any infected victim. 
    \item \textit{Fog Node Alerts:} 
    To minimize community transmission, we introduce automatic risk checker in public places such as shopping malls and office buildings. As there is a chance of revealing the user identity, we introduce \emph{time delay} and \emph{minimum entry} of people before broadcasting simple alert messages. These messages only request users to take precautions; do not reveal any RUERC or risk radius.

\end{enumerate}




\subsection{System Components}
Our framework has four
% \Razon{In the starter of Framework Design, "three" major component is mention} \Shanto{Just Fixed, good observation :D}
major components: a mobile application that broadcasts its RUERC, and stores received RUERCs from nearby devices. The ARC checks for infected cases and broadcast alerts in organization building. The SUDUN uploads data from the device of infected cases. Finally, a central cloud application integrates all these mobile and fog nodes and manages collected data. 

\subsubsection{Mobile Application}
Users download the application from the google play store or govt server and install it in the mobile device. The application broadcasts its RUERC and receives RUERC of other devices around. It also detects the special predefined UERC broadcasted by Automatic Risk Checker (ARC) and alerts the user about an infected or suspected case around.

% \vspace{1.5mm}
\subsubsection{Automatic Risk checker (IoT/Fog) (ARC)}
This fog device is set inside the hospital, shopping mall, educational institutes, and in all government-supervised organizations where there is a possibility of community transmission. The fog can receive the RUERC of the mobile devices within the Bluetooth range and interacts with cloud service to detect any infected or suspected victim. If any RUERC is found as an infected or suspected victim, it broadcasts a specific UERC throughout the place. The mobile application near the fog receives this specific UERC and alerts the user about the risk. As the fog node is registered via cloud fleet management service, the ARC node can be monitored in real-time. Thus it allows identifying any ARC node with a high rate of COVID-19 affected patient's presence. If the number of infected patients or the number of suspected patients gets higher than a predefined maximum threshold value per hour, it automatically generates emergency alert service to the organization's authority by sending emails and messages. It informs the nearby health authorities as well. The notification is broadcast only when there are at least $5$ persons within the range of ARC to ensure the privacy of the infected victim. On the contrary, the notification is not sent instantly when the ARC identifies an infected or suspected victim. It notifies the users after a certain period, which ensures the identity of the infected or suspected victim is not disclosed to others.

% \vspace{1.5mm}
% \Aron{do not add spaces manually before every subsubsection, use the titlespacing command from titlesec package}
\subsubsection{Suspected User Data Uploader Node (IoT/Fog) (SUDUN)}
% \Razon{Shovon vai, I have made some changes here, please verify the technical points.}
These fog nodes are similar to ARC and are set at the health centers or the COVID-19 test centers. When a test center reports a positive test result, the infected person can voluntarily allow the application to enable uploading its RUERC list from the privacy dashboard and keep the mobile phone within the range of a SUDUN.
% \Razon{Shanto vai, please review this line.} 
A SUDUN automatically connects with the user's device and fetches the list of stored lists of hashed RUERC from the device. Here, we enable monitoring each SUDUN using a cloud dashboard on a real-time basis. Additionally, the infected victim can also upload the RUERC list by using the mobile application and an internet connection without the help of a SUDUN.

% \vspace{1.5mm}
\subsubsection{Cloud/Server}
The government provided secure data storage and computing server. Receiving and storing data from SUDUN, mining to predict essential patterns or super spreaders, computing to provide required information to ARC, and handling standard authentication to maintain security and privacy are its primary responsibilities.





% \subsection{Application}
% \subsubsection{User Role}
% \begin{enumerate}[i.]
%     \item \textbf{General User (GU):} 
%     This user will generate a UERC against his/her phone number and NID and receive other’s UERC. The primary users of the system.
    
%     \item \textbf{Risk Checker (RC):} 
%     It is a proposed alternative of \snippet{ARC} and integrated inside the application of the system. After installing the app, the user can choose between GU and RC. This part is only for institutions, authorized by the Government. If anyone wants to be RC, they have to be registered and will have a Government provided ID.
%     It is more of a manual part where the mobile / NID needs to be input and the entry is required to be controlled manually. This user requires two-authentication as well.
    
%     \item \textbf{Authority Application (AP):}
%     This is the authority who has the password to send the collected data of a case to the server. The authority puts the password and an OTP is sent to corresponding authority against the UERC of that case. While entering the OTP, the data will be sent to the server. This is the proposed alternative to \snippet{ADR}.
% \end{enumerate}





\subsection{System Workflow}
\subsubsection{User Registration}
Initially, users need to register in the cloud using mobile number, age group, and postal code. The mobile number field is mandatory; however, the age group and postal code are optional. The Cloud Application generates and sends a One Time Password(OTP) to the user-submitted mobile number through SMS. Then the user enters the OTP in the mobile application, and the app sends the OTP to Cloud. The cloud application matches the user sent OTP, with the generated one. If both matches, the cloud application generates a UERC for the user and send it back to the user installed mobile app. 
%On the contrary, it shows an error response to the user about mismatched OTP and the user is being prompted to retry the registration process. 
Finally, the mobile app stores the UERC in encrypted format in the user device and then proceeds to scan IDs broadcasted by other users. The user device itself broadcasts a rotational UERC (derived from the initial UERC) as well. Figure~\ref{fig:registration} presents the complete registration process.

% \begin{enumerate}[i.]
    % \item The user provides a phone number and national ID (NID).
    % \item The Mobile Application sends the phone number and NID to Cloud Application.
    % \item The Cloud Application verifies user's identity from Government owned people's identity verification service using REST Api call.
    % \item If the identity verification returns a success response, then the Cloud Application generates and sends an One Time Password(OTP) to user submitted mobile number through SMS. If the identity verification fails, then the user is informed about the failed event and being prompted to retry the registration process.
    % \item User enters the OTP in the Mobile Application and the Mobile Application sends the OTP to Cloud Application.
    % \item The Cloud Application matches the user sent OTP with the generated one. If both are matched then it generates a UERC for the user. The server returns the UERC to Mobile Application if the OTP is matched. On the contrary, it shows an error response to the user about mismatched OTP and the user is being prompted to retry the registration process.
    % \item On approval, the Mobile Application stores the UERC in encrypted format in the user mobile device and proceeds to scan.
% \end{enumerate}

\begin{figure}[!ht]
    \centering
    \includegraphics[width=.5\textwidth]{figures/registration.pdf}
    \caption{User Registration Process}
    \label{fig:registration}
\end{figure}

% \subsubsection{Permissions}
% \begin{enumerate}
%     \item The application shows a dialog consisting of the messages “Why user needs to ‘accept’ the access permission”.
%     \item User press ‘Okay’.
%     \item Permission dialog is prompt. 
%     \item On permission allowed, the application checks Bluetooth connectivity.
%     \item If the Bluetooth is turned off, the application asks the user to turn on the Bluetooth.
%     \item The application asks the user to add the app into whitelist so that the app can perform in a low energy state.
% \end{enumerate}

% \itodo{References:\\
% $https://www.mdpi.com/1424-8220/20/1/118/htm$\\
% $https://www.researchgate.net/profile/Xu_Jiuqiang/publication/220279158_Distance_measurement_model_based_on_RSSI_in_WSN/links/567ca73708aebccc4e0122e7.pdf$
% }
% RSSI shows the strength of the received signal. It depends on the power and chipset of the broadcasting device. It also depend
% \begin{enumerate}[i.]
%     \item Range: No standard range. Based on device power Tx and its chipset. Usually between 0 to -100.
%     \item Unit: dB.
%     \item The calculated distance from RSSI is not accurate but nearly acceptable.
%     \item To be careful, we will add 1 extra foot to the WHO suggested 6 feet to measure.
% \end{enumerate}

% \vspace{1.5mm}
\subsubsection{Key Generation}
Our framework generates Rotational UERC (RUERC) with an interval of two hours. A person is considered a suspect case if he stays nearby to an infected person for an hour. As the RUERC changes every two hours, possibly the users are supposed to receive more than one RUERC if they stay nearby longer than an hour (e.g., in case they are neighbors). Our mobile application ensures that even if a person comes in close at any minute, it will store individual key and compare against the timestamp. It increases the accuracy of finding contact without a rigorous need for computation. Moreover, the RUERC enhances the privacy of the user because always broadcasting the same UERC may result in wireless tracking.
While registering, the mobile unit receives a UERC from the cloud, and from this UERC, it generates RUERCs using the AES algorithm on each two-hour interval for the next 14 days. When two devices come close, they transmit and save these RUERCs. Figure~\ref{fig:key_gen_steps} presents the steps of RUERC generation.


\begin{figure}[!t]
    \centering
    \includegraphics[width=.5\textwidth]{figures/key_generation.pdf}
    \caption{Key Generation Steps}
    \label{fig:key_gen_steps}
\end{figure}







% \vspace{1.5mm}
\subsubsection{RUERC Scan Service}
% \begin{enumerate}[i.]
%     \item The app creates a new thread so that it doesn’t interrupt the main thread.
%     \item The app assigns the new thread to the service.
%     \item The service runs on that new thread in the background.
%     \item The app starts the scan service and sets a constant notification in the notification tray to indicate the user that “COVID Finder has a service running”.
% \end{enumerate}
Scan service allows the application to run in the background. It creates a new thread so that the user does not feel any obstacle while using other mobile apps. 
%A notification is required to set on top of the device indicating the user that the app is running in background. 
The user has the privilege to stop and then restart running the service at any time. Scanning and advertising RUERC, creating files, and saving data are its primary responsibilities.

Scan service uses Bluetooth Low Energy (BLE) technology to share RUERC between two mobile devices. 
%BLE was introduced with Bluetooth 4.0 \cite{ble2}. 
The BLE consumes significantly less power to communicate, control, and monitor IoT devices. It uses \snippet{central} and \snippet{peripherals}, which define a network called piconet \cite{ble1}. Central scans for the advertisement and peripheral makes the advertisement. In our framework, the advertisement consists of the defined RUERC.
The Generic Attribute Profile (GATT) is designed to send and receive short pieces of data known as "attributes," and it is built on Attribute Protocol (ATT), which uses 128-bit unique ID~\cite{ble1}. In our framework, to maintain the minimal data collection policy and preserve device power, we are omitting the use of GATT and ATT. We are using emph{peripheral} to transmit the RUERC and the \emph{central} to scan these RUERCs. While scanning, we filter these RUERCs with our \emph{suspect filtering algorithm} and save accordingly.

\subsubsection{RSSI}
The framework uses a Received Signal Strength Indicator (RSSI) to identify the distance between devices. RSSI shows the strength of the received signal. It is calculated in dB and depends on the power and chipset of the broadcasting device. It also depends on the transmitting medium. If there is any obstacle between the receiver and the sender, the signal strength will decrease, so the RSSI. Therefore, for a different manufacturer, the value of RSSI in a specific medium shows different values. However, for a particular manufacturer, RSSI shows the intensity of the signal strength. 
RSSI does not provide the accurate distance but using path loss model \cite{kumar2009distance}, an approximate distance can be found,
% \Aron{will be more readable if you denote multiplication explicitly using $\cdot$}
% \Aron{also, format log as $\log$}
\begin{equation*}
    RSSI = -10 \cdot n \cdot \log_{10}(d) + C
\end{equation*}
Here, \textit{n} is the path loss exponent that depends on the transmitting medium, \textit{d} is the distance, and \textit{C} is a constant.



% \subsubsection{Scan service components}
% Scan Service manages the files, prepare BLE and scanning components and handle the scanning life-cycle. It has different components to operate these tasks.
% \begin{enumerate}[i.]

% \vspace{1.5mm}
\subsubsection{RUERC Storage in mobile device}
To maintain user privacy, the mobile application creates two files in the internal storage of the mobile device. Even the user does not have permission to access these files. When the peripheral receives any signal, one file temporarily stores this signal information, and other stores the information of the filtered signal. When the device comes within the range of SUDUN, the signal information of the filtered file is sent to SUDUN or directly to the cloud to perform self-check.
% \end{enumerate}


% \vspace{1.5mm}
\subsubsection{Suspect Filtering}
According to CDC, a distance of six feet between the case and contact is safe to maintain~\cite{CDC:online}. A person is considered a contact if he/she is within six feet for at least fifteen minutes or is within the proximity for an hour~\cite{COVID19C58:online}.
The scan service scans all the RUERCs within the range of Bluetooth. However, considering the rules mentioned above, continuous scanning is unnecessary as it causes battery and memory consumption. Therefore, the scanning service scans for $700 ms$ with three minutes interval. We develop our suspect filtering algorithm considering these factors so that the power and memory consumption is minimal, and identifying suspects is more accurate.

There are two types of files in the mobile device. One contains all the signal information (RUERC, distance, and timestamp) it receives from nearby devices on each interval. If any received signal passes the filtering conditions, associate information (RUERC, distance, timestamp, and duration) is stored in another file. This file is called the \emph{final file} and sent to the cloud once the user is found COVID-19 positive. A specific RUERC is stored in the final file only once a day. Here, the suspect filtering algorithm is shown in Algorithm~\ref{algo:suspect_filter}.


% \begin{table}[!ht]
% \centering
% \caption{Variables used in our Algorithm}
% \label{tab:algo_var}
% \begin{tabular}{|c|l|}
% \hline
% \textbf{Variable} & \multicolumn{1}{c|}{\textbf{Definition}} \\ \hline\hline
%     $Suspected$     &   Set of suspected cases                              \\ \hline
%          &                                 \\ \hline
%          &                                 \\ \hline
%          &                                 \\ \hline
%          &                                 \\ \hline
% \end{tabular}
% \end{table}

\begin{algorithm}[!ht]
\DontPrintSemicolon
  
%   \KwInput{Your Input}
%   \KwOutput{Your output}
%   \KwData{Testing set $x$}
\tcc{
$T_F$ = Temporary File, $F_F$ = Final File,\\
$T_c$ = Current Time, $T_r$ = Registerd Time,\\
$T_{15}$ = 15 minutes, $T_{60}$ = 60 Minutes,\\
$D_c$ = Current Distance, $D_r$ = Registered Distance, 
$D$ = Standard Distance (6 Feet), $C_t$ = Contact, $C_s$ = Case,
$S_{c}S_{n}$ = Scanned Signal, $R_{c}S_{n}$ = Recorded Signal in $T_F$,\\
$ASU$ = ARC specific UERC, $RSU$ = Risk specific UERC, \\
$SSU$ = SUDUN specific UERC
}

\ForEach{Signal in $R_{c}S_{n}$}    
        { 
        	 \If{$S_{c}S_{n}$.contains(Signal) == false}
                {$R_{c}S_{n}$.remove(Signal)}
        }
        
\ForEach{Signal in $S_{c}S_{n}$}    
        { 
        	 \If{Signal.RUERC == self.RUERC OR Signal.RUERC == $ASU$}
        	    {
        	        return
        	    }
        	 \If{Signal.RUERC == $RSU$}
        	    {
        	        showRiskAlert()
        	        return
        	    }
        	 \If{Signal.RUERC == $SSU$}
        	    {
        	        sendFileToSUDUN()
        	        return
        	    }
        	 \If{$R_{c}S_{n}$.contains(Signal) == false}
                {$R_{c}S_{n}$.add(Signal)}
            \Else
            {
            	Set $T_c$ = Signal.time, $T_r$ = $R_{c}S_{n}$.get(Signal.RUERC).time, $D_c$ = Signal.distance, $D_r$ = $R_{c}S_{n}$.get(Signal.RUERC).distance\;
            	
            	\If{$D_c <= D$ AND $D_r <= D$}
                {
                    \If{$T_c - T_r >= T_{15}$}
                    {
                    $C_t$ = Signal\;
                    \If{($F_F$.contains($C_t$) AND $F_F.get(C_t).time.date == C_t.time.date$) OR isUserConsentToStoreData == false}
                    {
                        return
                    }
				    $F_F$.add($C_t$)\;
				    }
				    
				    \Else
                    {
                    	$D_r$ = $D_c$\;
                    }
                }
                
                \ElseIf{$T_c - T_r >= T_{60}$}
                {
                	$C_t$ = Signal\;
                	\If{($F_F$.contains($C_t$) AND $F_F.get(C_t).time.date == C_t.time.date$) OR isUserConsentToStoreData == false}
                    {
                        return
                    }
			        $F_F$.add($C_t$)\;
                }
                
                \Else
                    {
                    	$D_r = D_c$\;
                    }
            }
        }


\caption{Filtering suspected RUERC in mobile application}
\label{algo:suspect_filter}
\end{algorithm}





% \subsection{Activity Diagram}
% \itodo{Need an activity diagram}
\subsection{Data Processing}
The framework is divided into three data processing layers to preserve user privacy and restrict access to data in various processes. Users can register to the system using a public communication process via mobile application. In this same access layer, the test centers can send the test results using RESTful API services through HTTPs protocol. The users can connect ARC and SUDUN fog node through the BLE protocol and send data to fog nodes. The computation and initial screening of user-uploaded data in fog nodes is done in a protected network layer. The APIs which are consumed by user mobile applications, test centers, and fog nodes are also in this layer. The main data processor consisting of a set of application nodes resides in a protected network, and users cannot access the data processor directly. The processed data is stored in data storage, which is configured in a restricted private subnet. This subnet can only be accessed from the ancestor private subnet, not from any public subnet. The data layer is protected from SQL injection as it is not directly connected through any user entries. Figure~\ref{fig:process_flow_diagram} displays the process flow diagram.



\begin{figure}[!ht]
    \centering
    \includegraphics[width=0.49\textwidth]{figures/original_pfd.pdf}
    \caption{Process Flow Diagram with Privacy and Security Boundaries}
    \label{fig:process_flow_diagram}
\end{figure}



==> privacy-preserving fog-mobile framework/tables/comparison.tex <==
\begin{table*}[!t]
\caption{Comparison between Existing Solutions and Our Solution}
\label{tab:comparison}
\resizebox{\textwidth}{!}{ 
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|}
\hline
 \multirow{2}{*}{\diagbox[innerwidth = 8em,
            height = 9.5ex]{\textbf{Frameworks}}{\textbf{Features}}} & \multicolumn{5}{c|}{\textbf{Privacy-preserving Approaches}}   & \multicolumn{2}{c|}{\textbf{Fog Computing}} & \multicolumn{3}{c|}{\textbf{Design Approaches}}  \\ \cline{2-11}
 & Volunatary & \begin{tabular}[c]{@{}c@{}}Data Usage\\ Limitation\end{tabular} & \begin{tabular}[c]{@{}c@{}}Data\\ Destruction\end{tabular} & \begin{tabular}[c]{@{}c@{}}Minimal Data\\ Collection\end{tabular} & Transparency & \begin{tabular}[c]{@{}c@{}}Risk\\Check\end{tabular} &  \begin{tabular}[c]{@{}c@{}}Infected/Suspected\\Data Upload\end{tabular} & \begin{tabular}[c]{@{}c@{}}Temporary\\BLE ID\end{tabular} & \begin{tabular}[c]{@{}c@{}}No Location\\Tracking\end{tabular} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Minimal\\Internet Use\end{tabular}} \\ \hline\hline
 Tracetogether &  \checkmark  &  \checkmark  & \checkmark  &  \checkmark  &  \checkmark  &
 \textbf{x}   &  \textbf{x}      &       \checkmark       &      \checkmark                                                  &   \checkmark \\ \hline
 MPC  Solution & \checkmark & \checkmark & \textbf{x} & \checkmark & \textbf{x} &  \textbf{x} & \textbf{x} & \checkmark & \checkmark & \textbf{x} \\ 
 \hline
 Matching  Solution &  \textbf{x}  &  \checkmark   &  \textbf{x}   &  \textbf{x}  & \textbf{x}  & \textbf{x}  & \textbf{x}  &  \checkmark & \checkmark  & \checkmark   \\ \hline
 DP-3T  Solution &  \checkmark  &  \checkmark  &  \checkmark   &  \checkmark  & \checkmark   &  \textbf{x}  &  \textbf{x}  &  \checkmark   & \checkmark & N/A \\ \hline
 COVIDSafe & \checkmark  & \checkmark  & \checkmark & \checkmark  &  \textbf{x}   &  \textbf{x}  &  \textbf{x}  & \textbf{x}  &     \checkmark &  \checkmark  \\ \hline
 PPMF &  \checkmark  &  \checkmark  & \checkmark  &  \checkmark  &  \checkmark &  \checkmark  & \checkmark  &  \checkmark & \checkmark  &  \checkmark   \\ \hline
\end{tabular}
}
\end{table*}
